MobileDev-Bench: A Benchmark for Issue Resolution in Mobile Application Development

Large language models (LLMs) have shown strong performance on automated software engineering tasks, yet existing benchmarks focus primarily on library-style repositories, leaving mobile application development largely unexplored despite its framework-specific build systems, heterogeneous artifact types, and coordinated multi-file fix requirements. We introduce MobileDev-Bench, a benchmark comprising 407 real-world issue-resolution tasks collected from 19 production mobile applications spanning Android Native (Java/Kotlin), React Native (TypeScript), and Flutter (Dart). Each task pairs a verified developer-reported issue with executable test patches, enabling fully automated validation of model-generated fixes within mobile build environments. The benchmark exhibits substantially greater patch complexity than prior benchmarks: fixes modify 12.9 files and 334.6 lines on average, and 41% of instances require coordinated changes across multiple artifact types, such as source, build configuration, and resource files. Evaluation of four frontier LLMs (Claude Sonnet 4.5, Qwen3-Coder, GPT-5.2, and Gemini 2.5 Flash) yields end-to-end resolution rates of only 3.23% - 4.23% under automated retrieval and at most 5.69% under oracle retrieval, well below resolution rates reported on existing benchmarks. We release MobileDev-Bench with task instances, an evaluation harness, and containerized environments to support reproducible research on AI-assisted mobile application development.

==> baseline.tex <==
\section{Baseline Results}
\label{sec:baseline}
\subsection{Model Candidates}
\begin{itemize}
    \item Overview of tested LLMs (GPT-4, Code Llama, Codex, etc.).
    \item Model configurations and hyperparameters.
\end{itemize}

\subsection{Quantitative Findings}
\begin{itemize}
    \item Performance metrics across different PR types (bug fixes vs.\ features).
    \item Breakdown by language or framework (Swift, Kotlin, Java).
\end{itemize}

\subsection{Qualitative Analysis}
\begin{itemize}
    \item Common error modes (e.g., incomplete fixes, missing platform details).
    \item Case studies of successful solutions vs.\ partial solutions.
\end{itemize}

==> conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}

This paper presents MobileDev-Bench, an evaluation benchmark specifically designed for assessing large language models on mobile application development tasks. We detailed the construction process and conducted a comprehensive statistical analysis of the dataset. Additionally, we have open-sourced the dataset, evaluation Docker environment, and leaderboard. In the future, we plan to expand the benchmark to include additional mobile platforms such as iOS (Swift and Objective-C), cross-platform frameworks like Flutter and React Native, while also continuing to improve the quality and coverage of the existing Android datasets.




==> dataset.tex <==
\section{MobileDev-Bench}
\label{sec:dataset}

MobileDev-Bench is a comprehensive benchmark for evaluating large language models' capabilities in mobile software engineering tasks, specifically focused on Android application development. The benchmark consists of [XXX] task instances derived from real-world GitHub pull requests across popular Android projects including WordPress, Thunderbird, Element-X, and others. This section describes the construction pipeline, validation methodology, and key characteristics of MobileDev-Bench.


\subsection{Benchmark Construction}

The construction of MobileDev-Bench follows a rigorous five-phase pipeline designed to ensure high-quality, executable, and challenging task instances that reflect real-world mobile development scenarios. As illustrated in Figure [X], the process progresses from repository selection through automated and manual validation stages.

\subsubsection{Phase 1: Repository Selection}

\subsubsection{Phase 2: Pull Request Crawling}

For each selected repository, we systematically collect pull requests using the GitHub API with specific filtering criteria designed to identify suitable issue-resolution tasks:

Merged Status. Only PRs with "merged" status are considered, indicating that the code changes were reviewed, approved, and integrated into the main codebase. This ensures that the gold patches represent validated solutions to real problems.

Issue Linkage. PRs must explicitly resolve one or more GitHub issues, identified through standard conventions such as "fixes \#123", "closes \#456", or "resolves \#789" in PR titles, bodies, or commit messages. This linkage provides the problem statement and contextual information necessary for task formulation.

Test Modification Requirement. Following the SWE-bench methodology, we require that PRs include modifications to test files (identified by paths containing "test", "androidTest", or "Test" keywords). This ensures that each task instance has associated tests for automated validation. However, unlike traditional software benchmarks, Android projects often separate unit tests from instrumentation tests, requiring specialized handling during validation.

Build Variant Awareness. Android projects frequently use multiple build variants (debug/release) and product flavors (free/paid/dev). We analyze build.gradle files to identify the primary variant used in CI/CD pipelines and ensure compatibility with the PR's test suite.

\subsubsection{Phase 3: Task Instance Construction}

\subsubsection{Phase 4: Environment Determination and Execution-Based Validation}
The validation phase ensures that each task instance is executable and exhibits the expected test behavior. This is the most technically complex phase, particularly for Android projects which present unique challenges compared to traditional software benchmarks.



MobileDev-Bench represents a significant step toward comprehensive evaluation of LLM capabilities in mobile software engineering. By focusing on real-world Android development tasks with rigorous validation, the benchmark provides a challenging and realistic testbed for advancing AI-assisted mobile development tools.



\subsection{Benchmark Characteristics and Statistics}

% \begin{itemize}
%     \item Selection of apps (diversity, popularity, categories).
%     \item Criteria for including/excluding certain repositories.
% \end{itemize}

% \subsection{Pull Request Extraction}
% \begin{itemize}
%     \item Methods to obtain PRs, issues, code diffs, test results, developer discussions.
%     \item Tooling or scripts used for data collection.
% \end{itemize}

% \subsection{Annotation Schema}
% \begin{itemize}
%     \item Taxonomy (bug fixes, features, refactoring, UI changes).
%     \item Success/failure labeling (merged vs.\ closed).
%     \item Metadata (code complexity, test coverage, device-specific issues, etc.).
% \end{itemize}

% \subsection{Dataset Statistics}
% \begin{itemize}
%     \item Overall PR count and distribution across categories.
%     \item Code changes (e.g., lines of code, language used, frameworks).
%     \item Average discussion length, test coverage data.
% \end{itemize}


% Regular Test Transitions (when builds succeed in both phases):
% % \begin{itemize}
% %     \item fail_to_pass_tests: Tests that failed \→ now pass
% %     \item pass_to_pass_tests: Tests that passed \→ still pass
% %     \item pass_to_fail_tests: Tests that passed \→ now fail
% %     \item fail_to_fail_tests: Tests that failed \→ still fail
% % \end{itemize}

% Build-Related Transitions (when build status changes):
% % \begin{itemize}
% %     \item build_to_pass_tests: Build failed \→ build succeeds, tests pass
% %     \item build_to_fail_tests: Build failed \→ build succeeds, tests fail
% %     \item pass_to_build_tests: Tests passed \→ build now fails
% %     \item build_to_build_tests: Build failed \→ build still fails
% % \end{itemize}


% \subsection{Instance Validation}

% For each set of task instances, we carry out the following steps:

% % 1. Create Android Build Environments.

% % All tasks can be run using the base mingc/android-build-box:latest image
% % from which different containers can be created based on JDK version (from gradle.properties or build.gradle), Gradle version (gradle/wrapper/gradle-wrapper.properties), Android SDK version (compileSdkVersion), Build tools version (buildToolsVersion) and NDK version (if applicable).

% - Using the mingc/android-build-box:latest docker image, create android build Environments/containers.

% - Environments must be customized based on compatible java/jdk version, gradle version, sdk version, ndk version (if applicable), and org.gradle.jvmargs or default to Xmx4096m  i.e. the script automatically parses the necessary build files (and .gradle files) to detect the build configurations.

% - Remove any file changes and checkout the task instance’s base commit. This sets the repository to codebase C.

% - Ensure tests are only ran for one test variant if the repo has multiple variants (preferrably the debug variant).

% - Apply the test patch T to codebase C.

% - Run the testing script, determined from test patch T , to generate test result logs logpre (part f).

% - Apply the solution δ patch to the codebase C with tests T.

% - Run the testing script (from part f again) to generate test result logs logpost.


==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}


Our evaluation reveals overall resolution rates of 3.23\%–4.23\% (Agentless) and 1.98\%–5.69\% (Oracle) on {\benchmark}. Three architectural properties of mobile development explain this low performance. First, \textit{multi-artifact coordination}: models achieve 1.63x success on single-artifact tasks but only 0.09x on multi-artifact tasks requiring synchronization across source code, resources, build configurations, and manifests. Second, \textit{framework-mediated execution}: platform lifecycles obscure control flow from static analysis. Third, \textit{cross-module dependencies}: recall drops from 35--55\% on single-file tasks to 7--9\% on multi-file tasks (6--10 files), and further to 2--3\% on large-scale tasks (11+ files).

Localization is the primary bottleneck. File-level recall of 13.8--18.6\% imposes a hard ceiling on resolution rates. For mobile development, the challenge lies not in generating correct patches but in identifying which files need modification. This finding suggests research should prioritize multi-file dependency tracing, artifact-aware retrieval, and framework-specific reasoning over patch generation improvements.

Resolution rates decline monotonically with file count: single-file tasks achieve 12.7 to 15.5\% resolution, 2--3 file tasks drop to 2.2--4.5\%, mid-complexity tasks (4--10 files) fall to 0--3.8\%, and tasks with 11+ files yield 0\% across all models. This pattern suggests models struggle with \textit{architectural complexity} (interconnected changes across heterogeneous components) rather than raw file count.




\section{Future Work}
Our findings suggest three high-priority research directions. First, given that localization is the primary bottleneck, techniques combining semantic search with static analysis for multi-file dependency tracing warrant immediate investigation. Second, repository-specific success patterns hint that certain architectural characteristics aid automated repair; systematically analyzing what makes codebases "LLM-friendly" could inform both tool design and best practices. Third, mobile issues often include screenshots and crash logs; evaluating multi-modal models' ability to ground repairs in visual artifacts may improve UI-related bug localization. Extending to iOS, developing framework-aware representations encoding lifecycle semantics, and testing iterative agentic workflows provide additional promising directions.


==> eval.tex <==
\section{Evaluation Methodology}
\label{sec:eval-method}
\subsection{Experimental Setup}
\begin{itemize}
    \item How to run models in zero-shot vs.\ few-shot modes.
    \item Prompt templates or instructions provided to models.
    \item Build environment: automated CI, test harness, etc.
\end{itemize}

\subsection{Evaluation Metrics}
\begin{itemize}
    \item \textbf{Automated:} Test pass/fail, code diff correctness, coverage.
    \item \textbf{Human Judgments:} Code readability, alignment with developer guidelines, maintainability.
    \item \textbf{Aggregate Analysis:} Efficiency (iterations needed), partial fixes, etc.
\end{itemize}



==> figure_repository_distribution.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{figures/repository_distribution_pie.pdf}
\vspace{-0.3cm}
\caption{Distribution of MobileDev-Bench's 596 instances across 18 repositories. Numbers in parentheses indicate instance counts per repository. \todo{make labels more legible}}
\label{fig:repository-distribution}
\end{figure}


==> intro.tex <==
\section{Introduction}
\label{sec:introduction}

Mobile applications serve billions of users globally, driving demand for efficient development practices and automated assistance tools. Recent advances in large language models (LLMs) such as GPT-4~\citep{openai2023gpt4}, Claude~\citep{anthropic2023claude}, and Code Llama~\citep{roziere2023code} have shown promise in code generation and program repair, particularly through benchmarks like SWE-bench~\citep{jimenez2024swebench} that evaluate issue resolution on real-world repositories. However, existing benchmarks focus primarily on general-purpose languages and web frameworks, overlooking the unique challenges of mobile development: platform-specific APIs, declarative UI frameworks, lifecycle management, asynchronous programming patterns, and framework-specific build systems.

Mobile development presents distinct complexities absent from traditional software engineering. Applications rely heavily on platform APIs for device features (camera, GPS, sensors), implement sophisticated UIs with gesture handling and navigation, manage extensive asynchronous operations for network and database access, and require understanding of framework-specific testing paradigms. Build systems involve intricate configurations with Gradle (Android), npm (React Native), or pub (Flutter), while testing spans unit tests, widget/component tests, and instrumentation tests on emulators or devices. These challenges demand specialized knowledge that differs significantly from backend or CLI development.

We introduce \textbf{MobileDev-Bench}, a benchmark of 595 real-world issue resolution tasks from 18 production mobile applications across three major frameworks: Android Native (Java/Kotlin with 77.5\% of instances), React Native (TypeScript with 8.9\%), and Flutter (Dart with 10.6\%), plus legacy Java (3.0\%). Each task represents a verified GitHub issue with an associated merged pull request, validated through comprehensive test execution. We ensure quality by executing test suites in two configurations—test patch only and complete fix—tracking behavioral transitions to verify genuine issue resolution without regressions.

We evaluate four state-of-the-art models on MobileDev-Bench: GPT-5.2, Claude Sonnet 4.5, Gemini Flash 2.5, and Qwen3-Coder. Our analysis reveals significant challenges current LLMs face with framework-specific APIs, state management patterns, and asynchronous operations unique to mobile platforms.

Our contributions are:

\begin{itemize}
    \item A benchmark of 595 mobile development tasks spanning three frameworks with reproducible environments and automated validation.
    \item First systematic evaluation of LLMs across diverse mobile paradigms—native (imperative), React Native (component-based), and Flutter (widget-based).
    \item Rigorous behavioral test validation ensuring high-quality, resolvable instances.
    \item Comprehensive baseline evaluation revealing performance gaps and mobile-specific challenges.
    \item Public release of tasks, evaluation harness, and Docker environments for reproducible research.
\end{itemize}


==> related.tex <==
% \section{Related Work}
% \label{sec:related}

% \textbf{Code Generation Benchmarks} Early code generation benchmarks focused on function-level synthesis tasks. HumanEval~\citep{chen2021evaluating} and MBPP~\citep{austin2021program} evaluate models on standalone programming problems that can be solved with a few lines of code. While these benchmarks established fundamental evaluation methodologies, they do not capture the complexity of real-world software development, where engineers must navigate large codebases, understand inter-file dependencies, and integrate changes across multiple modules. RepoBench~\citep{liu2023repobench} addresses repository-level code auto-completion by evaluating models' ability to retrieve relevant cross-file context and predict code given multi-file dependencies. The benchmark demonstrates that effectively utilizing cross-file context is crucial for realistic code completion. However, RepoBench focuses on next-line prediction rather than complete issue resolution, limiting its scope to a narrower set of software engineering tasks. JavaBench~\citep{cao2024javabench} targets project-level Java code generation with emphasis on Object-Oriented Programming (OOP) features including encapsulation, inheritance, and polymorphism. The benchmark contains 389 methods across 106 classes in four educational projects, achieving 92\% test coverage. Despite being project-level, JavaBench focuses on educational assignments rather than real-world open-source repositories, and does not evaluate issue resolution or bug fixing capabilities. Results show that LLMs achieve at most 41.17\% Pass@5 in test-wise evaluation, significantly below the 90.93\% average of undergraduate students, revealing substantial gaps in project-level OOP understanding.

% \textbf{Repository-Level Issue Resolution} SWE-bench~\citep{jimenez2024swebench} introduced a paradigm shift by evaluating models on repository-level issue resolution using real-world GitHub issues. The benchmark contains 2,294 task instances from 12 popular Python repositories, spanning library projects in data science, web development, and scientific computing. Each instance includes an issue description, a codebase snapshot at the pre-fix commit, and test cases that fail before the fix and pass after. Models must generate patches that resolve the issue without introducing regressions. Initial results showed that Claude 2 with BM25 retrieval resolved only 1.96\% of issues, highlighting the substantial difficulty of real-world software engineering tasks. SWE-bench Verified~\citep{jimenez2024swebench} addresses quality concerns through manual verification, selecting 500 instances with clear issue descriptions and appropriate test coverage. The human annotation process filters for instances where (1) issue descriptions are sufficiently clear, (2) test coverage adequately evaluates solutions, and (3) no major flaws exist. Within one year of release, the resolution rate on SWE-bench Verified increased from 0.40\% to 65.40\%, demonstrating rapid progress on carefully curated instances while highlighting the importance of data quality for reliable evaluation.

% Multi-SWE-bench~\citep{zan2024multiswebench} extends issue resolution evaluation to seven programming languages: Java, TypeScript, JavaScript, Go, Rust, C, and C++. The benchmark contains 1,632 human-validated GitHub issues across these languages, constructed through a systematic five-phase pipeline involving repository selection, pull request crawling, environment determination via Docker, pull request filtering based on test outcomes, and rigorous manual verification. The multilingual expansion revealed that techniques successful on Python do not necessarily generalize, with different languages exhibiting distinct failure patterns related to their programming paradigms, tooling ecosystems, and runtime behaviors. For instance, statically-typed languages like Java and C++ introduce unique compilation challenges, while dynamically-typed JavaScript presents different debugging and testing patterns. SWE-bench-java-verified~\citep{zan2024swebenchjava} provides 91 manually verified Java instances across six repositories including data serialization libraries (Jackson), web services frameworks (Dubbo), and container tools (Jib). During construction, the authors identified several infrastructure challenges when adapting the SWE-bench pipeline, including base commit crawling errors due to improper branch handling, redundant repository and dependency downloads across Docker containers, and compilation failures when applying incremental patches. While these challenges are not inherently Java-specific, they became particularly evident in Java projects due to the ecosystem's reliance on build tools like Maven and Gradle, which have more complex dependency management compared to Python's pip-based system. SWE-PolyBench~\citep{oviedo2024swepolybench} examines task complexity and compositional reasoning across 2,110 samples in four languages (Java, JavaScript, Python, and TypeScript) from 21 repositories. The key finding is that issues requiring edits to multiple files are substantially more challenging. SWE-PolyBench exhibits 63\% more files requiring modification per task compared to SWE-bench. The benchmark reveals that compositional reasoning, specifically understanding how changes in one part of a codebase affect other parts, remains a critical weakness for current LLMs. Analysis shows that while models can handle localized changes, they struggle with cross-module dependencies and maintaining consistency across file boundaries.

% \textbf{Limitations and the Mobile Development Gap} Despite substantial progress in software engineering benchmarks, several critical limitations persist. First, there is severe language imbalance. According to JavaBench, 95.8\% of existing benchmarks focus on Python, leaving other ecosystems underexplored. Second, task granularity remains concentrated at function or statement level (over 83\% of benchmarks), while real-world development increasingly involves navigating complex multi-module architectures. Third, existing benchmarks primarily assess general programming skills without evaluating platform-specific expertise required for specialized domains. Most critically, mobile development remains almost entirely absent from comprehensive LLM evaluation. While Multi-SWE-bench includes some Android repositories and SWE-bench Multimodal~\citep{yang2024swebenchmultimodal} incorporates visual elements from frontend tasks, no existing benchmark provides evaluation specifically designed for mobile development with its unique characteristics.

% Android projects rely on Gradle's intricate multi-module architecture with build variants (debug, release, flavors), annotation processing, and incremental compilation. Most benchmarks use straightforward build processes (pip for Python, Maven for Java) that do not capture this complexity. Mobile development requires deep understanding of dependency injection frameworks (Dagger/Hilt), reactive programming patterns (Coroutines, RxJava), lifecycle management (Activity/Fragment lifecycles), and Android-specific libraries. Existing benchmarks focus on algorithmic correctness rather than platform-specific design patterns. The transition from Java to Kotlin as Android's preferred language, combined with mixed-language codebases, introduces unique challenges that pure-language benchmarks cannot capture. While SWE-bench and its variants filter out instances with compilation failures, real-world mobile development frequently encounters such issues due to complex dependency injection, multi-module structures, and annotation processing. Infrastructure that handles compilation failures through techniques like automated stub generation is crucial for realistic evaluation.

% MobileDev-Bench addresses these gaps by providing the first comprehensive benchmark specifically designed for mobile software engineering. We focus on real-world Android applications with characteristic complexity: multi-module Gradle projects, Kotlin/Java interoperability, dependency injection frameworks, and platform-specific APIs. Our evaluation infrastructure includes sophisticated handling of compilation failures, proper management of build variants and test configurations, and fine-grained measurement of test state transitions (fail-to-pass, pass-to-pass, build-to-pass) that capture the nuances of mobile software quality assurance.


\section{Related Work}
\label{sec:related}

\textbf{Code Generation Benchmarks} Early benchmarks like HumanEval~\citep{chen2021humaneval} and MBPP~\citep{austin2021mbpp} evaluate models on standalone function-level problems solvable in a few lines of code. While foundational, they fail to capture real-world complexity where engineers navigate large codebases and manage inter-file dependencies. RepoBench~\citep{liu2023repobench} addresses repository-level code auto-completion, evaluating cross-file context retrieval and prediction, but focuses on next-line prediction rather than complete issue resolution. JavaBench~\citep{cao2024javabench} targets project-level Java code generation emphasizing OOP features (encapsulation, inheritance, polymorphism) across 389 methods in 106 classes. Despite 92\% test coverage, LLMs achieve only 41.17\% Pass@5 versus 90.93\% for undergraduate students, revealing significant gaps in project-level understanding.

\textbf{Repository-Level Issue Resolution} SWE-bench~\citep{jimenez2024swe} introduced a paradigm shift by evaluating models on repository-level issue resolution using real-world GitHub issues from Python repositories. Models generate patches evaluated against failing tests that must pass without introducing regressions. Initial results showed Claude 2 resolved only 1.96\% of issues. SWE-bench Verified~\citep{jimenez2024swebench-verified} manually curated 500 instances with clear descriptions and appropriate test coverage, achieving 65.40\% resolution within one year. Multi-SWE-bench~\citep{jain2024multi-swe-bench} extends evaluation to seven languages (Java, TypeScript, JavaScript, Go, Rust, C, C++) with 1,632 human-validated issues. The multilingual expansion revealed that Python-successful techniques do not generalize, with statically-typed languages introducing unique compilation challenges. SWE-bench-java-verified~\citep{2024swebenchjava} provides 91 Java instances across six repositories, encountering infrastructure challenges when adapting the pipeline, particularly around Maven/Gradle build complexity. SWE-PolyBench~\citep{rashid2025swepolybench} examines compositional reasoning across 2,110 samples, finding that multi-file edits are substantially harder with 63\% more files requiring modification versus SWE-bench. Models struggle with cross-module dependencies and maintaining consistency across file boundaries.

\textbf{The Mobile Development Gap} Despite substantial progress in software engineering benchmarks, several critical limitations persist. First, severe language imbalance exists with 95.8\% of benchmarks focusing on Python~\citep{cao2024javabench}. Second, task granularity concentrates at function/statement level (over 83\%), missing complex multi-module architectures. Third, benchmarks assess general programming without platform-specific expertise. Most critically, mobile development remains almost entirely absent. While Multi-SWE-bench includes some Android repositories and SWE-bench Multimodal~\citep{yang2024swebenchmultimodal} incorporates visual elements, no benchmark targets mobile-specific characteristics. Android projects use Gradle's multi-module architecture with build variants, annotation processing, and incremental compilation that straightforward build processes (pip, Maven) do not capture. Mobile development demands understanding of dependency injection (Dagger/Hilt), reactive patterns (Coroutines, RxJava), lifecycle management (Activity/Fragment), and platform-specific libraries. The Java-to-Kotlin transition with mixed codebases introduces challenges pure-language benchmarks miss. Existing benchmarks filter out compilation failures, yet mobile development frequently encounters such issues through complex dependency injection and annotation processing.

MobileDev-Bench addresses these gaps as the first comprehensive mobile software engineering benchmark, focusing on real-world Android applications with multi-module Gradle projects, Kotlin/Java interoperability, dependency injection frameworks, and platform-specific APIs. Our infrastructure handles compilation failures, manages build variants and test configurations, and measures fine-grained test state transitions (fail-to-pass, pass-to-pass, build-to-pass).

==> table_annotation_summary.tex <==
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{0.95}
\begin{tabular}{@{} l r r @{\quad\quad} l r r @{}}
\toprule
\multicolumn{3}{c}{\textit{Problem Statement Clarity (560 candidates)}}
  & \multicolumn{3}{c}{\textit{Unit-Test Coverage Adequacy (560 candidates)}} \\
\cmidrule(r){1-3}\cmidrule(l){4-6}
\textbf{Label} & \textbf{N} & \textbf{\%}
  & \textbf{Label} & \textbf{N} & \textbf{\%} \\
\midrule
0: well-specified              & 297 & 53.0 & 0: comprehensive              & 384 & 68.6 \\
1: minor ambiguity             & 165 & 29.5 & 1: mostly adequate            &  68 & 12.1 \\
2: vague \textbf{(excl.)}      &  64 & 11.4 & 2: reasonable gaps \textbf{(excl.)} & 63 & 11.2 \\
3: insufficient \textbf{(excl.)} & 34 &  6.1 & 3: misaligned \textbf{(excl.)} & 45 &  8.0 \\
\midrule
\multicolumn{3}{c}{\textit{Task Difficulty (415 verified)}}
  & \multicolumn{3}{c}{\textit{Issue Type (415 verified)}} \\
\cmidrule(r){1-3}\cmidrule(l){4-6}
\textbf{Level} & \textbf{N} & \textbf{\%}
  & \textbf{Type} & \textbf{N} & \textbf{\%} \\
\midrule
$<$15 min                      & 139 & 33.5 & Bug Fix                       & 180 & 43.4 \\
15 min--1 hr                   & 140 & 33.7 & New Feature                   & 152 & 36.6 \\
1--4 hrs                       &  82 & 19.8 & Feature Optimisation          &  83 & 20.0 \\
$>$4 hrs                       &  54 & 13.0 &                               &     &      \\
\midrule
\multicolumn{6}{@{}l}{Excluded: 98 (PS score $\geq 2$) $+$ 108 (TC score $\geq 2$)
  $-$ 39 (both) $=$ \textbf{176 total}; \quad verified benchmark: \textbf{415 instances}.} \\
\bottomrule
\end{tabular}
\caption{Manual annotation statistics. The upper panel shows score distributions for
problem-statement clarity (PS) and unit-test coverage adequacy (TC) across 560
execution-validated candidates; scores $\geq 2$ trigger exclusion.
The lower panel characterises the 415 verified instances by estimated resolution
difficulty and issue type.}
\label{tab:annotation-summary}
\end{table*}


==> table_artifact_types.tex <==
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\caption{Artifact type distribution in MobileDev-Bench fix patches. ``\% inst.'' is the percentage of instances modifying at least one file of that type; ``Avg. files'' is the average number of such files per instance across all instances.}
\label{tab:artifact-types}
\begin{tabular}{lrrrrrr}
\toprule
& \multicolumn{2}{c}{\textbf{Overall}} & \multicolumn{4}{c}{\textbf{\% instances by language}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-7}
\textbf{Type} & \textbf{\% inst.} & \textbf{Avg. files} & \textbf{Kt} & \textbf{Dart} & \textbf{TS} & \textbf{Java} \\
\midrule
Source   & 99.6 & 11.5 & 99.5 & 100.0 & 100.0 & 100.0 \\
Resource & 21.1 &  1.9 & 24.1 &   0.0 &  12.2 &  63.6 \\
i18n     & 21.1 &  1.1 & 20.4 &  18.8 &  22.4 &  54.5 \\
Build    & 20.5 &  0.6 & 23.2 &   0.0 &  26.5 &   9.1 \\
Manifest &  7.9 &  0.2 &  5.3 &   1.6 &  38.8 &   9.1 \\
Config   &  5.7 &  0.1 &  2.5 &   1.6 &  40.8 &   0.0 \\
Docs     & 10.9 &  0.2 & 10.8 &   1.6 &  26.5 &   0.0 \\
\bottomrule
\end{tabular}
\end{table*}


==> table_benchmark_comparison.tex <==
\begin{table}[t]
\centering
\footnotesize
\caption{Comparison of Software Engineering Benchmarks. Multi-SWE-bench covers 7 languages (Java, TypeScript, JavaScript, Go, Rust, C, C++). MobileDev-Bench covers 4 languages (Kotlin, Dart, TypeScript, Java).}
\begin{tabular}{lccc}
\toprule
\textbf{Benchmark} & \textbf{Lang.} & \textbf{Mobile} & \textbf{Build Systems} \\
\midrule
SWE-bench & Python & \ding{55} & Pip \\
Multi-SWE-bench & Multi & \ding{55} & Mixed \\
SWE-bench Java & Java & \ding{55} & Maven/Gradle \\
MobileDev-Bench & Multi & \ding{51} & Gradle/Npm/Pub \\
\bottomrule
\end{tabular}
\label{tab:benchmark-comparison-simple}
\end{table}

